Story Point Effort Estimation by Text Level Graph Neural Network

Estimating the software projects' efforts developed by agile methods is important for project managers or technical leads. It provides a summary as a first view of how many hours and developers are required to complete the tasks. There are research works on automatic predicting the software efforts, including Term Frequency Inverse Document Frequency (TFIDF) as the traditional approach for this problem. Graph Neural Network is a new approach that has been applied in Natural Language Processing for text classification. The advantages of Graph Neural Network are based on the ability to learn information via graph data structure, which has more representations such as the relationships between words compared to approaches of vectorizing sequence of words. In this paper, we show the potential and possible challenges of Graph Neural Network text classification in story point level estimation. By the experiments, we show that the GNN Text Level Classification can achieve as high accuracy as about 80 percent for story points level classification, which is comparable to the traditional approach. We also analyze the GNN approach and point out several current disadvantages that the GNN approach can improve for this problem or other problems in software engineering.

==> openProblems.tex <==
\section{Open Problems and Analysis}
Although we have potential accuracy compared to the TFIDF-RF approach, there are several current challenges that we can improve in future works.
\subsection{From Text Classification to Text Regression} 
The TextLevelGNN approach \cite{008_TextLevelGNN} is applicable in text or issue classification. Though the space of story point value is not in uniform distribution, the story point estimation should be considered as the text regression problem instead of classification. We study other works in Software Engineering that applied GNN. We see that most of them focus on the classification or code generation instead of regression such as \cite{005_allamanisgraph}. There are a few of problems in SE can be formalized as regression problem such as project assignment scoring \cite{020_ProgramAssignmentScoring} and Github star project prediction \cite{021_GithubStarPrediction}, however, none of them applied GNN as solutions. We studied several works on graph regression in NLP and see that most of them focus on dataset in different research area such as image processing \cite{022_GNNOverview}. 

\textbf{Considering story points as labels for classification} A simple solution to convert from classification to regression problem is that we consider the story points themselves as labels for classification. Next, we evaluate the correctness of output by Mean Absolute Error (MAE). We compare with the traditional approach TFIDF with Random Forest Regression (TFIDF-RFR). The result which is shown in Table \ref{tblAccuracy}, reveals the fact that the TextLevelGNN approach achieves higher MAE than the BOW-RFR approach. It means the TextLevelGNN didn't perform as good as the traditional approach with this simple solution for converting from classification to regression problem. In the upcoming work, we intend to change the mechanism in \cite{008_TextLevelGNN} to regression learning to support for story point estimation.

% \begin{table}
% \centering
% \caption{Results on the Mean Absolute Error of TF-IDF-RFR and TextLevel-GNN for Story Point Regression Estimation}
% \label{tblMAE}
% \begin{tabular}{|r|l|r|r|}
% \hline
% \multicolumn{1}{|c|}{\textbf{No}} & \multicolumn{1}{c|}{\textbf{Software}} & \multicolumn{1}{c|}{\textbf{TF-IDF-RFR}} & \multicolumn{1}{c|}{\textbf{TextLevel-GNN}} \\ \hline
% 1                                 & appceleratorstudio                     & 1.83                                     & 1.67                                        \\ \hline
% 2                                 & aptanastudio                           & 2.96                                     & 3.57                                        \\ \hline
% 3                                 & bamboo                                 & 1.34                                     & 0.87                                        \\ \hline
% 4                                 & clover                                 & 2.98                                     & 4.06                                        \\ \hline
% 5                                 & datamanagement                         & 4.78                                     & 6.90                                        \\ \hline
% 6                                 & duracloud                              & 0.96                                     & 0.93                                        \\ \hline
% 7                                 & jirasoftware                           & 2.1                                      & 1.76                                        \\ \hline
% 8                                 & mesos                                  & 1.31                                     & 1.30                                        \\ \hline
% 9                                 & moodle                                 & 10.2                                     & 11.19                                       \\ \hline
% 10                                & mule                                   & 2.31                                     & 2.49                                        \\ \hline
% 11                                & mulestudio                             & 3.29                                     & 3.90                                        \\ \hline
% 12                                & springxd                               & 1.98                                     & 1.90                                        \\ \hline
% 13                                & talenddataquality                      & 4.49                                     & 4.10                                        \\ \hline
% 14                                & talendesb                              & 0.86                                     & 0.87                                        \\ \hline
% 15                                & titanium                               & 2.58                                     & 2.79                                        \\ \hline
% 16                                & usergrid                               & 1.19                                     & 1.22                                        \\ \hline
% \multicolumn{1}{|l|}{}            & \textbf{Average MAE}                   & 2.82                                     & 3.09                                        \\ \hline
% \end{tabular}
% \end{table}

\subsection{Optimization in Running Time and Graph Complexity} 
We see that the running time in the training of your approach is longer than the traditional work. The BOW-RF approach requires \textbf{4} minutes to complete the training step, while the TextLevelGNN requires about \textbf{25} minutes for the same tasks of training on 16 projects of \cite{004_DeepLearningSPEstimation}. The testing step achieves almost the same running time for the TFIDF-RF approach and our approach. We study the result and see that one problem due to long training time is the number of edges in our graph is usually high, which can be more than 500000 edges in complicated projects such as $memos$. In future work, we can optimize the running time by simplifying the graph in which we highlight important information. First, along with making edges between adjacent words, we can filter and making edges between important words instead. Second, we can build the graph based on the information from the part of speech tagger to avoid non-necessary information.

\textbf{Analysis on the scale of graph.} To study how the complexity can affect the performance of the training process, we analyze the nodes, the edges, the size (number of issues for training) and compare with similar metrics on the popular natural text dataset $R8$ which was used in the work \cite{008_TextLevelGNN}. We have some observations. First, the size of 16 projects is smaller than the R8 dataset. The number of issues for each project ranges from over 200 to 3000. Second, the number of nodes in the R8 dataset is about 3000, which is lower than some projects like $datamanagement, memos$, or $talendesb$. It means that there are more new words inside each issue instead of a standard NLP text dataset. We study some issues and we see that the description of issues is usually longer than the description that the combination of title and descriptions can be more than 10 sentences. This fact of causing the risk of out-of-vocabulary words that didn't appear in the standard vector corpus Glove used in \cite{008_TextLevelGNN}. We can improve this challenge by building a new Glove representation trained from the context of issues' description. Third, the number of edges is much larger than the number of nodes. This is because the mechanism of making edges between a word and neighbor words in the offset $w=20$ causes the exponential of the edges. Similarly, the number of edges provided in the $R8$ dataset is high which is about $1.3$ million edges. In the issues dataset, the project that has the highest number of edges is $memos$ project, due to the complexity of long issues' description. The project that has the least number of edges is the $jirasoftware$ project, which can be due to the compact number of training records. Forth, for the running time, the running time for each project ranges from about 9 seconds to 370 seconds, which is comparable with the $R8$ dataset.

% \centering
% \caption{Analysis on scale of graphs extracted from training data}
% \label{tblAnalysisResult}

\begin{table}
\centering
\caption{Analysis on scale of graphs extracted from training data}
\label{tblAnalysisResult}

\begin{tabular}{|l|l|r|r|r|r|}
\hline
\multicolumn{1}{|c|}{\textbf{Paper}} & \multicolumn{1}{c|}{\textbf{Project}} & \multicolumn{1}{c|}{\textbf{Size}} & \multicolumn{1}{c|}{\textbf{Nodes}} & \multicolumn{1}{c|}{\textbf{Edges}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Train\\ Time \\ (second)\end{tabular}}} \\ \hline
{[}3{]}                              & appceleratorstudio                    & 1868                               & 14969                               & 1218745                             & 239                                                                                            \\ \hline
{[}3{]}                              & aptanastudio                          & 530                                & 8211                                & 545099                              & 40                                                                                             \\ \hline
{[}3{]}                              & bamboo                                & 332                                & 6175                                & 297828                              & 20                                                                                             \\ \hline
{[}3{]}                              & clover                                & 245                                & 5227                                & 339562                              & 14                                                                                             \\ \hline
\textbf{{[}3{]}}                     & \textbf{datamanagement}               & \textbf{2986}                      & \textbf{18490}                      & \textbf{1618297}                    & \textbf{370}                                                                                   \\ \hline
{[}3{]}                              & duracloud                             & 425                                & 3793                                & 289685                              & 22                                                                                             \\ \hline
{[}3{]}                              & jirasoftware                          & 224                                & 2339                                & 151170                              & 9                                                                                              \\ \hline
\textbf{{[}3{]}}                     & \textbf{mesos}                        & \textbf{1075}                      & \textbf{25494}                      & \textbf{1698010}                    & \textbf{104}                                                                                   \\ \hline
{[}3{]}                              & moodle                                & 745                                & 8468                                & 696113                              & 74                                                                                             \\ \hline
{[}3{]}                              & mule                                  & 568                                & 6133                                & 437088                              & 30                                                                                             \\ \hline
{[}3{]}                              & mulestudio                            & 468                                & 4316                                & 309768                              & 23                                                                                             \\ \hline
{[}3{]}                              & springxd                              & 2256                               & 17198                               & 1194025                             & 144                                                                                            \\ \hline
{[}3{]}                              & talenddataquality                     & 883                                & 7324                                & 445830                              & 92                                                                                             \\ \hline
\textbf{{[}3{]}}                     & \textbf{talendesb}                    & \textbf{555}                       & \textbf{8766}                       & \textbf{591293}                     & \textbf{35}                                                                                    \\ \hline
{[}3{]}                              & titanium                              & 1440                               & 23989                               & 1728925                             & 310                                                                                            \\ \hline
{[}3{]}                              & usergrid                              & 308                                & 4114                                & 218491                              & 18                                                                                             \\ \hline
{[}7{]}                              & R8 dataset                            & 4937                               & 2923                                & 1380208                             & 821                                                                                            \\ \hline
\end{tabular}
\end{table}

\textbf{Simplifying the graph of issues by verb and noun.} We analyze the potential of simplifying the input text as issue by filtering its words' roles in part of speech tagging by an experiment that its results are shown in Table \ref{tblSimplifyAccuracy}. In this study, we filter the words that are verbs and nouns and remove all words in other tags of the issue. We run the experiment on the $datamanagement$ project, we called this configuration as $verbNounFilter$. The results show that the accuracy is \textbf{61.72\%} on this project, compared to \textbf{60.6\%} with the normal text without filter. More over, the training time and the graph complexity are alleviate. Though this is a very beginning and heuristic strategy to simplify the textual content, it shows the potential of simplifying the graph that focused on important part of speech tags.

\begin{table}
\centering
\caption{Accuracy on simplifying the graph in verb-noun format in datamanagement project}
\label{tblSimplifyAccuracy}
\begin{tabular}{|l|r|r|}
\hline
\multicolumn{1}{|c|}{\textbf{Metric}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Raw \\ issue\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Filter \\ Verb-Noun\end{tabular}}} \\ \hline
nodes                                 & 18490                                                                              & \textbf{2986}                                                                             \\ \hline
edges                                 & 1618297                                                                            & \textbf{10309}                                                                            \\ \hline
training time                         & 370                                                                                & \textbf{209}                                                                              \\ \hline
accuracy                              & 60.60\%                                                                            & \textbf{61.72\%}                                                                          \\ \hline
\end{tabular}
\end{table}

\textbf{Sensitivity on window size.} We study the impact of window size to the number of edges and the classification accuracy by the sensitivity experiment by changing window size to one of following sizes: $[2,5,10,20,50,100]$. We evaluate on projects $jirasoftware$ and $clover$. The impact of window size to number of edges is shown in Table \ref{tblSensitivityEdgeSize}, which shows the highly increasing of edges when we increase the window size. The accuracy experiment is shown in Figure \ref{figSensitivityWindow}. We can see that too big window size can cause the decrease of the accuracy, possibly due to many non-useful edges of constructed graph.

\begin{figure}
        \center{\includegraphics[width=\linewidth]
        {images/sensitivityWindow.png}}
        \caption{Sensitivity experiment on projects jirasoftware and clover with window size as $[2,5,10,20,50,100]$}
        \label{figSensitivityWindow} 
\end{figure}

\begin{table}
\centering
\caption{Number of edges of projects jirasoftware and clover with window size as $[2,5,10,20,50,100]$}
\label{tblSensitivityEdgeSize}
\begin{tabular}{|l|r|r|}
\hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}window \\ size\end{tabular}}} & \multicolumn{1}{c|}{\textbf{jirasoftware}} & \multicolumn{1}{c|}{\textbf{clover}} \\ \hline
w=2                                                                                   & 22511                                      & 48658                                \\ \hline
w=5                                                                                   & 58752                                      & 124600                               \\ \hline
w=10                                                                                  & 99626                                      & 213987                               \\ \hline
w=20                                                                                  & 151170                                     & 339562                               \\ \hline
w=50                                                                                  & 229599                                     & 568997                               \\ \hline
w=100                                                                                 & 287869                                     & 772672                               \\ \hline
\end{tabular}
\end{table}
